Delay Closure of Observable Dynamics for the Heat Equation

We study finite-delay representations of point observables, which are solution values at selected spatial locations, for spatially discretized heat equations. We show that the observables satisfy closed dynamical systems whose evolution depends only on their own history, without requiring solution values elsewhere in the domain. Using semigroup properties, we analyze low-rank approximate closures that can use substantially fewer delay terms than the exact representation. We consider two computational approaches: direct least-squares fitting of delay coefficients from observable trajectories and shift-invert Krylov approximation of the semigroup using preconditioned linear solves. Numerical experiments for constant- and variable-coefficient heat equations in one, two, and three dimensions illustrate the effects of memory length and sensor information on prediction. The results are consistent with the theoretical analysis.

==> Tables/sensor_location_summary.tex <==
% Source: Old project Tables/table_q1_y_rollout_position_p_eps.tex
% and table_q3_y_rollout_position_p_eps.tex. Entries are exact min--max
% summaries of the supplied selected orders at the three shown tolerances.
\begin{table}[tb]
\centering
\caption{Ranges of the selected delay order over sensor placements in
the one-dimensional study: $20$ single-sensor locations and $10$
translated triplets. Each entry is the minimum--maximum range of
$r_\varepsilon(t)$ over configurations; a single number means that all
configurations give the same order. All configurations attain the
reported tolerances within $r\leq16$.}
\label{tab:sensor-location-summary}
\small
\begin{tabular}{ccccc}
\toprule
 & \multicolumn{2}{c}{One sensor} & \multicolumn{2}{c}{Three sensors}\\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}
$\varepsilon$ & $t=0.5$ & $t=1$ & $t=0.5$ & $t=1$\\
\midrule
$10^{-12}$ & 4 & 4 & 2 & 1--2 \\
$10^{-13}$ & 4 & 4 & 2 & 2 \\
$10^{-14}$ & 4--8 & 4--8 & 2 & 2 \\
\bottomrule
\end{tabular}
\end{table}

